$\ell_{\infty}$-Bounds of the MLE in the BTL Model under General Comparison Graphs

The Bradley-Terry-Luce (BTL) model is a popular statistical approach for estimating the global ranking of a collection of items using pairwise comparisons. To ensure accurate ranking, it is essential to obtain precise estimates of the model parameters in the $\ell_{\infty}$-loss. The difficulty of this task depends crucially on the topology of the pairwise comparison graph over the given items. However, beyond very few well-studied cases, such as the complete and Erd\"os-R\'enyi comparison graphs, little is known about the performance of the maximum likelihood estimator MLE) of the BTL model parameters in the $\ell_{\infty}$-loss under more general graph topologies. In this paper, we derive novel, general upper bounds on the $\ell_{\infty}$ estimation error of the BTL MLE that depend explicitly on the algebraic connectivity of the comparison graph, the maximal performance gap across items and the sample complexity. We demonstrate that the derived bounds perform well and in some cases are sharper compared to known results obtained using different loss functions and more restricted assumptions and graph topologies. We carefully compare our results to Yan et al. (2012), which is closest in spirit to our work. We further provide minimax lower bounds under $\ell_{\infty}$-error that nearly match the upper bounds over a class of sufficiently regular graph topologies. Finally, we study the implications of our $\ell_{\infty}$-bounds for efficient (offline) tournament design. We illustrate and discuss our findings through various examples and simulations.

==> Makefile <==
# Generic make file for LaTeX: requires GNU make

# Main compilation file for latex
MAINFILE = li_649.tex
SUPPFILE = li_649-supp.tex

.PHONY: all clean clean_adhoc fresh rem_zip supp uai_dir

fresh:
	make clean

main:
	latexmk -pdf -bibtex li_649.tex

supp:
	latexmk -pdf -bibtex li_649-supp.tex

uai_dir:
	rm -rf li_649
	mkdir -p li_649/latex
	@cp \
	$(MAINFILE:.tex=.aux) \
	$(MAINFILE:.tex=.log) \
	$(MAINFILE:.tex=.out) \
	$(MAINFILE:.tex=.pdf) \
	$(MAINFILE:.tex=.tex) \
	$(MAINFILE:.tex=.fdb_latexmk) \
	$(MAINFILE:.tex=.fls) \
	$(SUPPFILE:.tex=.aux) \
	$(SUPPFILE:.tex=.log) \
	$(SUPPFILE:.tex=.out) \
	$(SUPPFILE:.tex=.pdf) \
	$(SUPPFILE:.tex=.tex) \
	$(SUPPFILE:.tex=.fdb_latexmk) \
	$(SUPPFILE:.tex=.fls) \
	li_649/latex
	cp 000_custom_macros_comb.sty li_649/latex
	cp refs.bib li_649/latex
	cp -r figures li_649/latex/
	zip -r li_649.zip li_649/latex

clean_adhoc:
	find . -name '.DS_Store' -type f -delete
	find . -iname '*conflicted*.fls' -type f -delete
	find . -iname '*conflicted*.tex' -type f -delete
	find . -iname '*conflicted*.pdf' -type f -delete
	find . -iname '*conflicted*' -type f -delete
	rm -rf auto
	rm -rf "#Makefile#"
	rm -rf "#.Makefile"
	rm -rf *.synctex.gz
	rm -rf *.bbl
	rm -rf __latexindent_temp*

clean:
	@rm -f \
	$(MAINFILE:.tex=.aux) \
	$(MAINFILE:.tex=.log) \
	$(MAINFILE:.tex=.out) \
	$(MAINFILE:.tex=.pdf) \
	$(MAINFILE:.tex=.ps) \
	$(MAINFILE:.tex=.fdb_latexmk) \
	$(MAINFILE:.tex=.fls) \
	$(SUPPFILE:.tex=.aux) \
	$(SUPPFILE:.tex=.log) \
	$(SUPPFILE:.tex=.out) \
	$(SUPPFILE:.tex=.pdf) \
	$(SUPPFILE:.tex=.fdb_latexmk) \
	$(SUPPFILE:.tex=.fls)
	make clean_adhoc
	latexmk -c
	rm -rf li_649

rem_zip:
	rm -rf li_649.zip

all:
	rm -rf li_649
	make rem_zip
	make clean
	make main
	make supp
	make uai_dir
	make clean


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

